Adaptive Submodular Optimization under Matroid Constraints

Many important problems in discrete optimization require maximization of a monotonic submodular function subject to matroid constraints. For these problems, a simple greedy algorithm is guaranteed to obtain near-optimal solutions. In this article, we extend this classic result to a general class of adaptive optimization problems under partial observability, where each choice can depend on observations resulting from past choices. Specifically, we prove that a natural adaptive greedy algorithm provides a $1/(p+1)$ approximation for the problem of maximizing an adaptive monotone submodular function subject to $p$ matroid constraints, and more generally over arbitrary $p$-independence systems. We illustrate the usefulness of our result on a complex adaptive match-making application.

==> intro.tex <==
\section{Introduction} \label{sec:intro}
%
Submodular functions play an important role in discrete optimization.
Many important problems, such as facility location~\cite{nemhauser78}, coverage~\cite{wolsey82}, influence maximization~\cite{kempe03}, and experimental design~\cite{srinivas10gaussian} can be reduced to constrained maximization of a submodular set function.  Submodularity, informally, is an intuitive notion of diminishing  returns, which states that adding an element to a small set helps
 more than adding that same element to a larger (super-)set.  
While maximizing submodular functions in general is NP-hard, a
celebrated result of \mycitet{Nemhauser~\etal}{nemhauser78} shows that a
simple greedy algorithm is guaranteed to find a near-optimal solution
to the problem of maximizing a submodular function subject to
cardinality constraints; the value of the greedy solution obtains at
least a constant fraction of $(1-1/e)$ of the optimal value.
\mycitet{Nemhauser and Wolsey}{nemhauser78best} furthermore show that, in general, obtaining better approximation guarantees requires evaluating the objective function on an exponential number of sets. Beyond cardinality constraints, the greedy algorithm also obtains guarantees for maximizing a monotone submodular function subject to $p$ matroid constraints~\cite{fisher78}, and, more generally, $p$-independence systems~\cite{calinescu07}.  In both cases, the greedy algorithm  achieves at least a constant fraction of $1/(p+1)$ of the optimal value. 

Submodular optimization provides a unified framework for many
important non--adaptive optimization problems. In many practical
optimization problems, however, one needs to \emph{adaptively} make a
sequence of decisions, taking into account observations about the
outcomes of past decisions.  Often these outcomes are uncertain, and
one may only know a probability distribution over them.  Finding
optimal policies for decision making in such partially observable
stochastic optimization problems is notoriously intractable (see,
e.g., \cite{papadimitriou87complexity}).  
The classical notion of submodular set functions does not allow one to
handle such adaptive optimization problems. In recent
work~\cite{golovin10colt,golovin10adaptiveARXIV}, we 
%
%
introduced the concept of \emph{\term submodularity}, a natural generalization of submodular set functions to adaptive policies, and prove that if a partially observable stochastic optimization problem satisfies this property, a simple adaptive greedy
algorithm is guaranteed to obtain near-optimal solutions in the case of cardinality constraints.
The concept has several useful applications, including active learning,
machine diagnosis, adaptive viral marketing, and sensor placement~\cite{golovin10adaptiveARXIV,golovin10nips}. 


In this article, we prove that the adaptive greedy algorithm is
guaranteed to obtain a $1/(p+1)$-approximation for the more general problem of
maximizing an adaptive submodular function over $p$-independence systems
(and therefore subject to $p$ matroid constraints).  Our results
generalize those obtained by
\mycitet{Asadpour~\etal}{AsadpourNS08long}  for optimizing a
particular instance of adaptive submodular functions to a single
matroid constraint to arbitrary adaptive monotone submodular functions
and to arbitrary $p$-independence systems. We illustrate the
usefulness of this result on adaptive match--making problems such as
online dating.  We show that the constraint system in this application
is a $2$-independence system, and thus the adaptive greedy algorithm
provides a $1/3$-approximation.
%

%
%
%
%
%

%
%
%
%
%
%
%
%


%
%
%
%

